Cosmic Shear in Harmonic Space from the Dark Energy Survey Year 1 Data: Compatibility with Configuration Space Results

We perform a cosmic shear analysis in harmonic space using the first year of data collected by the Dark Energy Survey (DES-Y1). We measure the cosmic weak lensing shear power spectra using the Metacalibration catalogue and perform a likelihood analysis within the framework of CosmoSIS. We set scale cuts based on baryonic effects contamination and model redshift and shear calibration uncertainties as well as intrinsic alignments. We adopt as fiducial covariance matrix an analytical computation accounting for the mask geometry in the Gaussian term, including non-Gaussian contributions. A suite of 1200 lognormal simulations is used to validate the harmonic space pipeline and the covariance matrix. We perform a series of stress tests to gauge the robustness of the harmonic space analysis. Finally, we use the DES-Y1 pipeline in configuration space to perform a similar likelihood analysis and compare both results, demonstrating their compatibility in estimating the cosmological parameters $S_8$, $\sigma_8$ and $\Omega_m$. The methods implemented and validated in this paper will allow us to perform a consistent harmonic space analysis in the upcoming DES data.

==> Galaxy Shear in Harmonic Space (3)/affiliations.tex <==
\section*{Author Affiliations}
\label{app:affiliations}
$^{1}$ Instituto de F\'{i}sica Te\'orica, Universidade Estadual Paulista, S\~ao Paulo, Brazil\\
$^{2}$ Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{3}$ ICTP South American Institute for Fundamental Research\\ Instituto de F\'{\i}sica Te\'orica, Universidade Estadual Paulista, S\~ao Paulo, Brazil\\
$^{4}$ Departamento de F\'isica Matem\'atica, Instituto de F\'isica, Universidade de S\~ao Paulo, CP 66318, S\~ao Paulo, SP, 05314-970, Brazil\\
$^{5}$ Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA\\
$^{6}$ Department of Astronomy, University of California, Berkeley,  501 Campbell Hall, Berkeley, CA 94720, USA\\
$^{7}$ Department of Astronomy/Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA\\
$^{8}$ Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA\\
$^{9}$ Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{10}$ Department of Physics, Northeastern University, Boston, MA 02115, USA\\
$^{11}$ Laboratory of Astrophysics, \'Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Observatoire de Sauverny, 1290 Versoix, Switzerland\\
$^{12}$ Jodrell Bank Center for Astrophysics, School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, M13 9PL, UK\\
$^{13}$ California Institute of Technology, 1200 East California Blvd, MC 249-17, Pasadena, CA 91125, USA\\
$^{14}$ Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA\\
$^{15}$ Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA 94720, USA\\
$^{16}$ Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain\\
$^{17}$ Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain\\
$^{18}$ Faculty of Physics, Ludwig-Maximilians-Universit\"at, Scheinerstr. 1, 81679 Munich, Germany\\
$^{19}$ Department of Astronomy, University of Geneva, ch. d'\'Ecogia 16, CH-1290 Versoix, Switzerland\\
$^{20}$ Department of Applied Mathematics and Theoretical Physics, University of Cambridge, Cambridge CB3 0WA, UK\\
$^{21}$ Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA\\
$^{22}$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA\\
$^{23}$ Department of Physics, Carnegie Mellon University, Pittsburgh, Pennsylvania 15312, USA\\
$^{24}$ Brookhaven National Laboratory, Bldg 510, Upton, NY 11973, USA\\
$^{25}$ Department of Physics, Duke University Durham, NC 27708, USA\\
$^{26}$ Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain\\
$^{27}$ Institute for Astronomy, University of Edinburgh, Edinburgh EH9 3HJ, UK\\
$^{28}$ Cerro Tololo Inter-American Observatory, NSF's National Optical-Infrared Astronomy Research Laboratory, Casilla 603, La Serena, Chile\\
$^{29}$ Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA\\
$^{30}$ Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK\\
$^{31}$ CNRS, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{32}$ Sorbonne Universit\'es, UPMC Univ Paris 06, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{33}$ Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK\\
$^{34}$ SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA\\
$^{35}$ Center for Astrophysical Surveys, National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA\\
$^{36}$ Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA\\
$^{37}$ Physics Department, William Jewell College, Liberty, MO, 64068, USA\\
$^{38}$ Astronomy Unit, Department of Physics, University of Trieste, via Tiepolo 11, I-34131 Trieste, Italy\\
$^{39}$ INAF-Osservatorio Astronomico di Trieste, via G. B. Tiepolo 11, I-34143 Trieste, Italy\\
$^{40}$ Institute for Fundamental Physics of the Universe, Via Beirut 2, 34014 Trieste, Italy\\
$^{41}$ Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{42}$ Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{43}$ Hamburger Sternwarte, Universit\"{a}t Hamburg, Gojenbergsweg 112, 21029 Hamburg, Germany\\
$^{44}$ Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain\\
$^{45}$ Department of Physics, IIT Hyderabad, Kandi, Telangana 502285, India\\
$^{46}$ Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA\\
$^{47}$ Department of Astronomy, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{48}$ Institute of Theoretical Astrophysics, University of Oslo. P.O. Box 1029 Blindern, NO-0315 Oslo, Norway\\
$^{49}$ Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain\\
$^{50}$ School of Mathematics and Physics, University of Queensland,  Brisbane, QLD 4072, Australia\\
$^{51}$ Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{52}$ Department of Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{53}$ Center for Astrophysics $\vert$ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA\\
$^{54}$ Australian Astronomical Optics, Macquarie University, North Ryde, NSW 2113, Australia\\
$^{55}$ Lowell Observatory, 1400 Mars Hill Rd, Flagstaff, AZ 86001, USA\\
$^{56}$ George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA\\
$^{57}$ Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA\\
$^{58}$ Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain\\
$^{59}$ Physics Department, 2320 Chamberlin Hall, University of Wisconsin-Madison, 1150 University Avenue Madison, WI  53706-1390\\
$^{60}$ Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{61}$ School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK\\
$^{62}$ Computer Science and Mathematics Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831\\
$^{63}$ Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA\\
$^{64}$ Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany\\
$^{65}$ Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany\\
$^{66}$ Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK\\


==> Galaxy Shear in Harmonic Space (3)/authorlist.tex <==
% Author list file generated with: mkauthlist 1.2.4 
% mkauthlist -j mnras /home/hcamacho/Downloads/DES-2021-0650_author_list.csv 

\author[DES Collaboration]{
\parbox{\textwidth}{
\Large
H.~Camacho,$^{1,2}$\thanks{E-mail: hocamachoc@gmail.com (HC)}
F.~Andrade-Oliveira,$^{1,2}$
A.~Troja,$^{3,2}$
R.~Rosenfeld,$^{3,2}$\thanks{E-mail: rogerio.rosenfeld@gmail.com (RR)}
L.~Faga,$^{4,2}$
R.~Gomes,$^{4,2}$
C.~Doux,$^{5}$
X.~Fang,$^{6,7}$
M.~Lima,$^{4,2}$
V.~Miranda,$^{7}$
T.~F.~Eifler,$^{7,8}$
O.~Friedrich,$^{9}$
M.~Gatti,$^{5}$
G.~M.~Bernstein,$^{5}$
J.~Blazek,$^{10,11}$
S.~L.~Bridle,$^{12}$
A.~Choi,$^{13}$
C.~Davis,$^{14}$
J.~DeRose,$^{15}$
E.~Gaztanaga,$^{16,17}$
D.~Gruen,$^{18}$
W.~G.~Hartley,$^{19}$
B.~Hoyle,$^{18}$
M.~Jarvis,$^{5}$
N.~MacCrann,$^{20}$
J.~Prat,$^{21,22}$
M.~M.~Rau,$^{23}$
S.~Samuroff,$^{23}$
C.~S{\'a}nchez,$^{5}$
E.~Sheldon,$^{24}$
M.~A.~Troxel,$^{25}$
P.~Vielzeuf,$^{26}$
J.~Zuntz,$^{27}$
T.~M.~C.~Abbott,$^{28}$
M.~Aguena,$^{2}$
S.~Allam,$^{29}$
J.~Annis,$^{29}$
D.~Bacon,$^{30}$
E.~Bertin,$^{31,32}$
D.~Brooks,$^{33}$
D.~L.~Burke,$^{14,34}$
A.~Carnero~Rosell,$^{2}$
M.~Carrasco~Kind,$^{35,36}$
J.~Carretero,$^{26}$
F.~J.~Castander,$^{16,17}$
R.~Cawthon,$^{37}$
M.~Costanzi,$^{38,39,40}$
L.~N.~da Costa,$^{2,41}$
M.~E.~S.~Pereira,$^{42,43}$
J.~De~Vicente,$^{44}$
S.~Desai,$^{45}$
H.~T.~Diehl,$^{29}$
P.~Doel,$^{33}$
S.~Everett,$^{46}$
A.~E.~Evrard,$^{47,42}$
I.~Ferrero,$^{48}$
B.~Flaugher,$^{29}$
P.~Fosalba,$^{16,17}$
D.~Friedel,$^{35}$
J.~Frieman,$^{29,22}$
J.~Garc\'ia-Bellido,$^{49}$
D.~W.~Gerdes,$^{47,42}$
R.~A.~Gruendl,$^{35,36}$
J.~Gschwend,$^{2,41}$
G.~Gutierrez,$^{29}$
S.~R.~Hinton,$^{50}$
D.~L.~Hollowood,$^{46}$
K.~Honscheid,$^{51,52}$
D.~Huterer,$^{42}$
D.~J.~James,$^{53}$
K.~Kuehn,$^{54,55}$
N.~Kuropatkin,$^{29}$
O.~Lahav,$^{33}$
M.~A.~G.~Maia,$^{2,41}$
J.~L.~Marshall,$^{56}$
P.~Melchior,$^{57}$
F.~Menanteau,$^{35,36}$
R.~Miquel,$^{58,26}$
R.~Morgan,$^{59}$
F.~Paz-Chinch\'{o}n,$^{35,60}$
D.~Petravick,$^{35}$
A.~Pieres,$^{2,41}$
A.~A.~Plazas~Malag\'on,$^{57}$
K.~Reil,$^{34}$
M.~Rodriguez-Monroy,$^{44}$
E.~Sanchez,$^{44}$
V.~Scarpine,$^{29}$
M.~Schubnell,$^{42}$
S.~Serrano,$^{16,17}$
I.~Sevilla-Noarbe,$^{44}$
M.~Smith,$^{61}$
M.~Soares-Santos,$^{42}$
E.~Suchyta,$^{62}$
G.~Tarle,$^{42}$
D.~Thomas,$^{30}$
C.~To,$^{63,14,34}$
T.~N.~Varga,$^{64,65}$
J.~Weller,$^{64,65}$
and R.D.~Wilkinson$^{66}$
\begin{center} (DES Collaboration) \end{center}
}
}



==> Galaxy Shear in Harmonic Space (3)/introduction.tex <==
One of the consequences of the Theory of General Relativity is the precise prediction of the deflection of light due to the presence of matter in its path \citep{Einstein:1916vd}. This prediction was confirmed for the first time with the measurements of the positions of stars during a solar eclipse in 1919  by two expeditions, sent to Brazil and to the Principe Island \citep{Dyson:1920cwa}.
After roughly 100 years, and the enormous development of instrumental and theoretical methods, one is able to measure minute distortions in the shape of distant galaxies 
that provide information about the distribution of matter in the universe. These small distortions are called weak gravitational lensing, in opposition to strong gravitational lensing, when large distortions with multiple images of the same object are produced (for reviews see, e.g. \citet{Bartelmann:1999yn,2015RPPh...78h6901K,2017grle.book.....D,2018ARA&A..56..393M}).

Being a small effect, weak gravitational lensing can be detected only by capturing the images of a large sample of galaxies, usually called source galaxies, and performing shape measurements that can then be analyzed statistically. 
One of the most common ways to analyse weak lensing signals is by studying the correlation between shapes of two galaxies. This can be done in configuration space, with measurements of the two-point correlation functions, or in harmonic space and the corresponding measurement of the power spectra. Although 
they are both second order statistics and can be related by a Fourier transform, they probe scales differently, and so they behave differently to systematic effects and analysis choices. In practice, 
there are differences in the measurements and analyses that may yield different cosmological results from the configuration and harmonic space methods \citep{Hamana:2019etx}. 
In particular, the covariance matrix is known to be more diagonal (indicating less cross-correlations) in harmonic space than in configuration space due to the orthogonality of the spherical harmonics used to decompose the signal 
(see e.g., figure 2 in~\cite{y3-BAOkp}).
The consistency between cosmic shear analyses in configuration and harmonic space was recently investigated in \citet{Doux:2020duk},
using DES-Y3-like Gaussian mock catalogues and paying particular attention to the methodology of determining angular and multipole scale cuts in both cases.

In the past years, several collaborations reported results from weak gravitational lensing: the Deep Lens Survey (DLS)\footnote{\tt dls.physics.ucdavis.edu}, the Canada-France-Hawaii Telescope Lensing Survey (CFHTLenS)\footnote{\tt www.cfhtlens.org},  the Hyper Suprime-Cam Subaru Strategic Program (HSC-SSP)\footnote{\tt hsc.mtk.nao.ac.jp/ssp}, the Kilo-Degree Survey (KiDS)\footnote{\tt kids.strw.leidenuniv.nl} and the Dark Energy Survey (DES)\footnote{\tt www.darkenergysurvey.org}. 
DLS \citep{Jee:2012hr,Jee:2015jta} and CFHTLenS \citep{Joudaki:2016mvz} presented results from configuration space measurements whereas
HSC has performed the analysis both in harmonic space \citep{Hikage:2018qbn} and configuration space \citep{Hamana:2019etx}. KiDS has performed a cosmic shear analysis in configuration space for its 450 deg$^2$ survey \citep{Hildebrandt:2016iqg} and for its fourth  data release (KiDS-1000) a first comparison of configuration and harmonic space analyses was presented in \citep{Asgari:2020wuj} using bandpowers constructed from correlation functions, and more recently in \citep{2021arXiv211006947L} using the angular power spectrum forward modelling survey geometry effects, both showed excellent agreement.
For its first year of data (Y1), DES has presented a weak lensing analysis in configuration space only \citep{troxel_2018}. 

Two re-analyses of DES-Y1 weak gravitational lensing in combination with other experiments have been performed: KiDS-450 and DES-Y1 \citep{Joudaki:2019pmv}, and  DLS, CFHTLens, KiDS-450 and the DES Science Verification data \citep{Chang:2018rxd}. More recently, the DES-Y1 public data was used to perform a full 3x2pt analysis (the combination of shear, galaxy clustering and galaxy-galaxy lensing) in harmonic space with emphasis on the testing of a more sophisticated model for galaxy bias \citep{hadzhiyska2021hefty}. 

Consistency between different summary statistics analyses is expected when applied to the same data set.
As different statistics summarize information differently and could be sensitive to different systematic effects, consistency not only adds to the robustness of the different analyses and data reduction but also prevents ambiguity when comparing different data sets or analyses.
Nevertheless, recent studies have presented some tension on recovered parameters at the 0.5 to 1.5$\sigma$ between configuration and harmonic space analysis on the same data set.
See, e.g., cosmic shear analysis from the HSC \citep{Hamana:2019etx,Hikage:2018qbn,2022PASJ...74..488H}.
These tensions, although somehow small and understood in terms of the different scales probed, deserve consideration and showcase the importance of running both analyses in parallel for forthcoming galaxy surveys to understand better the capabilities and limitations of different two-point statistics.

The purpose of this paper is to complete the Y1 weak lensing analysis by presenting harmonic space results and comparing them to the configuration space ones. We measure the cosmic weak lensing shear power spectra  using the so-called \mcal catalogs\citep{mcal1,mcal2,zuntz:2017pso}. 
We perform a likelihood
analysis using the framework of CosmoSIS adopted by DES \citep{troxel_2018} assuming a fiducial $\Lambda$CDM cosmological model with parameters given in the Table \ref{tab:Parameters}. We use 1200 lognormal simulations originally developed for DES-Y1 \citep{krause:2017ekm} to validate
an analytical covariance matrix and scale cuts tested to curb the contributions from baryonic effects to the
shear power spectra. 
To demonstrate the compatibility between our analysis in harmonic space with the DES default analysis in configuration space, we run the DES-Y1 standard configuration space pipeline with a similar likelihood analysis methodology.
One of the main consequences of this work is to put forward a harmonic space analysis of galaxy shear validated with DES-Y1 data that justifies its adoption in an independent harmonic analysis with the DES-Y3 data \citep{2022MNRAS.tmp.1761D} and in the current analyses of the final six-years data set.

This paper is organized as follows.
Section~\ref{sec:formalism} reviews the basic theoretical modelling, including systematic effects such as redshift uncertainties, shear calibration and intrinsic alignments. In Section~\ref{sec:data} we describe the DES-Y1 data for the shear analysis presented here, Section~\ref{sec:Flask} presents the 1200 \flask lognormal mocks used to validate our pipeline and the analytical covariance matrix. Section~\ref{sec:methods} details our methodology including a discussion of the covariance matrix.
We perform likelihood analyses both in harmonic and configuration space and present our main results in Section~\ref{sec:results}, with some robustness tests shown in Section~\ref{sec:robustness}. We conclude in Section~\ref{sec:conclusions}. 


